Clustering-based Inference for Biomedical Entity Linking

Due to large number of entities in biomedical knowledge bases, only a small fraction of entities have corresponding labelled training data. This necessitates entity linking models which are able to link mentions of unseen entities using learned representations of entities. Previous approaches link each mention independently, ignoring the relationships within and across documents between the entity mentions. These relations can be very useful for linking mentions in biomedical text where linking decisions are often difficult due mentions having a generic or a highly specialized form. In this paper, we introduce a model in which linking decisions can be made not merely by linking to a knowledge base entity but also by grouping multiple mentions together via clustering and jointly making linking predictions. In experiments on the largest publicly available biomedical dataset, we improve the best independent prediction for entity linking by 3.0 points of accuracy, and our clustering-based inference model further improves entity linking by 2.3 points.

==> zz_fig_bc5cdr_e2e.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{cccc}
    \toprule
       & \bf Precision & \bf Recall & \bf F1\\
    \midrule
    \taggerOne   & XX  & XX & XX\\
    \independent & XX  & XX & XX\\
    \our (ours)& \textbf{XX} & \textbf{XX} & \textbf{XX}\\
    \bottomrule
    \end{tabular}
    \caption{End-to-end entity linking results on BC5CDR dataset for different inference methods using \taggerOne's mention detection.}
    \label{tab:bc5cdr_end2end}
\end{table}

==> zz_fig_bc5cdr_res.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lc|c c  @{}}
    \toprule
            & \bf Overall & \multicolumn{2}{c}{\bf Acc. on } \\
       & \bf Acc.   & \bf Seen & \bf Unseen \\
    \midrule
    \textsc{Independent} & 91.6  & 94.7 & 76.3 \\
    \our (ours)    & \textbf{92.0}  & \textbf{95.1} & \textbf{76.7} \\
    \bottomrule
    \end{tabular}
    \caption{Linking accuracy on BC5CDR dataset conditioned only on the gold span.}
    \label{tab:bc5cdr}
\end{table}

==> zz_fig_bc5cdr_res_gold_type.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{cc|cc}
    \toprule
                & \bf Overall & \multicolumn{2}{c}{\bf Acc. on } \\
       & \bf Acc.   & \bf Seen & \bf Unseen \\
    \midrule
    \taggerOne   & 90.3 & 94.5 & 71.4 \\
    \independent & 91.9  & 94.8 & 76.9 \\
    \our (ours)& \textbf{92.2} & \textbf{95.2} & \textbf{77.1}  \\
    \bottomrule
    \end{tabular}
    \caption{Linking accuracy on BC5CDR dataset conditioned on the gold mention type.}
    \label{tab:bc5cdr_gold_type}
\end{table}

==> zz_fig_bc5cdr_res_gold_type_no_single.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{cc|cc}
    \toprule
                & \bf Overall & \multicolumn{2}{c}{\bf Acc. on } \\
       & \bf Acc.   & \bf Seen & \bf Unseen \\
    \midrule
    \taggerOne   & 90.5 & 94.9 & 71.8 \\
    \independent & 92.0  & 95.4 & 76.0 \\
    \our (ours)& \textbf{92.9} & \textbf{96.3} & \textbf{76.9}  \\
    \bottomrule
    \end{tabular}
    \caption{Linking accuracy on BC5CDR dataset conditioned on the gold mention type with singleton mentions removed.}
    \label{tab:bc5cdr_gold_type_no_single}
\end{table}

==> zz_fig_bc5cdr_res_no_single.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lc|c c  @{}}
    \toprule
            & \bf Overall & \multicolumn{2}{c}{\bf Acc. on } \\
       & \bf Acc.   & \bf Seen & \bf Unseen \\
    \midrule
    \textsc{Independent} & 91.8  & 95.2 & 75.4 \\
    \our (ours)    & \textbf{92.4}  & \textbf{95.8} & \textbf{76.3} \\
    \bottomrule
    \end{tabular}
    \caption{Linking accuracy on BC5CDR dataset conditioned only on the gold span with singleton mentions removed.}
    \label{tab:bc5cdr_no_single}
\end{table}

==> zz_fig_bc5cdr_stats.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{p{2.5cm}c c c }
%     \toprule
%                             & \bf Train     & \bf Dev       & \bf Test \\
%     \midrule
%     \bf \# Mentions      & 18.0K   & 934    & 9.7K\\
%     \bf\# Entities      &   1.8K & 281 & 1.3K  \\
%     \bf \% Entities seen    &  100\%        & 80.1\% & 64.8\% \\
%     \bottomrule
%     \end{tabular}
%     \caption{Statistics train/dev/test split of BC5CDR dataset, including the percent of ground truth entities seen during training.}
%     \label{tab:bc5cdr_stats}
% \end{table}

==> zz_fig_binned_exp.tex <==
\begin{figure*}[ht]
\begin{subfigure}{.24\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{zz_fig.bc5cdr.untyped}  
  \caption{}
  \label{fig:bin_bc5cdr_untyped}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{zz_fig.bc5cdr.typed}  
  \caption{}
  \label{fig:bin_bc5cdr_typed}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{zz_fig.medmentions.untyped}  
  \caption{}
  \label{fig:bin_medmentions_untyped}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{zz_fig.medmentions.typed}  
  \caption{}
  \label{fig:bin_medmentions_typed}
\end{subfigure}
\caption{Put your caption here}
\label{fig:bin_exp}
\end{figure*}

==> zz_fig_medmentions_e2e.tex <==
%\begin{table}[]
%    \centering
%    \begin{tabular}{cccc}
%    \toprule
%       & \bf Precision & \bf Recall & \bf F1\\
%    \midrule
%    \taggerOne   & 47.1  & 44.8 & 45.9\\
%    \independent & 49.6  & 47.1 & 48.3\\
%    \our (ours)& \textbf{50.0} & \textbf{47.5} & \textbf{48.7}\\
%    \bottomrule
%    \end{tabular}
%    \caption{End-to-end entity linking results for different inference methods using \taggerOne's mention detection.}
%    \label{tab:medmentions_end2end}
%\end{table}
\begin{table}[]
    \centering
    \begin{tabular}{cccc}
    \toprule
       & \bf Precision & \bf Recall & \bf F1\\
    \midrule
    \taggerOne   & XX  & XX & XX\\
    \independent & XX  & XX & XX\\
    \our (ours)& \textbf{XX} & \textbf{XX} & \textbf{XX}\\
    \bottomrule
    \end{tabular}
    \caption{End-to-end entity linking results on MedMentions dataset for different inference methods using \taggerOne's mention detection.}
    \label{tab:medmentions_end2end}
\end{table}


==> zz_fig_medmentions_res_gold_type.tex <==
%\begin{table}[]
%    \centering
%    \begin{tabular}{cc|cc}
%    \toprule
%                & \bf Overall & \multicolumn{2}{c}{\bf Acc. on } \\
%       & \bf Acc.   & \bf Seen & \bf Unseen \\
%    \midrule
%    \taggerOne   & 73.8  & 78.2 & 58.8\\
%    \independent & 76.3  & 78.8 & 67.4 \\
%    \our (ours)& \textbf{78.1} & \textbf{80.7} & \textbf{69.2}  \\
%    \bottomrule
%    \end{tabular}
%    \caption{Linking accuracy on MedMentions dataset conditioned on the gold mention type.}
%    \label{tab:medmentions_gold_type}
%\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{cc|cc}
    \toprule
                & \bf Overall & \multicolumn{2}{c}{\bf Acc. on } \\
       & \bf Acc.   & \bf Seen & \bf Unseen \\
    \midrule
    \taggerOne   & 73.8  & 78.2 & 58.8\\
    \independent & 76.8  & 79.2 & 68.4 \\
    \our (ours)& \textbf{79.1} & \textbf{81.5} & \textbf{70.5}  \\
    \bottomrule
    \end{tabular}
    \caption{Linking accuracy on MedMentions dataset conditioned on the gold mention type.}
    \label{tab:medmentions_gold_type}
\end{table}



==> zz_fig_medmentions_res_gold_type_no_single.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{cc|cc}
    \toprule
                & \bf Overall & \multicolumn{2}{c}{\bf Acc. on } \\
       & \bf Acc.   & \bf Seen & \bf Unseen \\
    \midrule
    \taggerOne   & 74.1  & \textbf{81.2} & 53.7 \\
    \independent & 74.7  & 76.9 & 67.7 \\
    \our (ours)& \textbf{78.8} & 80.9 & \textbf{72.1}  \\
    \bottomrule
    \end{tabular}
    \caption{Linking accuracy on MedMentions dataset conditioned on the gold mention type removing singleton mentions.}
    \label{tab:medmentions_gold_type_no_single}
\end{table}

==> zz_fig_mentions_res.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lc|c c  @{}}
    \toprule
            & \bf Overall & \multicolumn{2}{c}{\bf Acc. on } \\
       & \bf Acc.   & \bf Seen & \bf Unseen \\
    \midrule
    \textsc{Independent} & 72.8  & 75.9 & 61.9 \\
    \our (ours)    & \textbf{74.1}  & \textbf{77.3} & \textbf{62.9} \\
    \bottomrule
    \end{tabular}
    \caption{Linking accuracy on MedMentions dataset conditioned only on the gold span.}
    \label{tab:medmentions}
\end{table}


==> zz_fig_mentions_res_no_single.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lc|c c  @{}}
    \toprule
            & \bf Overall & \multicolumn{2}{c}{\bf Acc. on } \\
       & \bf Acc.   & \bf Seen & \bf Unseen \\
    \midrule
    \textsc{Independent} & 71.1  & 73.9 & 62.2 \\
    \our (ours)    & \textbf{73.5}  & \textbf{76.3} & \textbf{64.4} \\
    \bottomrule
    \end{tabular}
    \caption{Linking accuracy on MedMentions dataset conditioned only on the gold span with singleton mentions removed.}
    \label{tab:medmentions_no_singles}
\end{table}

